Does context matter in digital pathology?

The development of Artificial Intelligence for healthcare is of great importance. Models can sometimes achieve even superior performance to human experts, however, they can reason based on spurious features. This is not acceptable to the experts as it is expected that the models catch the valid patterns in the data following domain expertise. In the work, we analyse whether Deep Learning (DL) models for vision follow the histopathologists' practice so that when diagnosing a part of a lesion, they take into account also the surrounding tissues which serve as context. It turns out that the performance of DL models significantly decreases when the amount of contextual information is limited, therefore contextual information is valuable at prediction time. Moreover, we show that the models sometimes behave in an unstable way as for some images, they change the predictions many times depending on the size of the context. It may suggest that partial contextual information can be misleading.

==> prev.tex <==
In the end, we will enrich our investigation by the use of eXplainable AI (XAI) tools to analyze where the model pays the most attention. 


In resized images, the center 

///////////////////////////
Swin model operates on 224x224, whereas Resnet on 96x96. For Swin we resized the input images, and so the center region changed the size. The size of context also changed, but for the comparison between Swin and conv, we rescaled the Swin size of context to the range corresponding to the ones in the case of conv. 

order of padding and resizing


\section{Appendices}

If your work needs an appendix, add it before the
``\verb|\end{document}|'' command at the conclusion of your source
document.

Start the appendix with the ``\verb|appendix|'' command:
% \begin{minted}{latex}
% \appendix
% \end{minted}
and note that in the appendix, sections are lettered, not
numbered. 

%%
%% The acknowledgments section is defined using the "acknowledgments" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.


%prevent overflowing URLs; suggested by Franck in
% https://tex.stackexchange.com/questions/636114/how-can-i-prevent-urls-in-an-eprint-field-from-overflowing-in-the-references-i/636172#636172



It turns out that {\color{red} convolutional models are more sensitive to the removal of contextual information. It is especially visible in the case of recall metrics which is }




##### ML for insights


\st{The general observation is that the performance results decrease with the limitation of the amount of contextual information. The bottom plots in Figure~\ref{fig:probs_4categories} suggest that some images }


////// CZY WSTAWIMY TABELĘ Z MIARAMI RÓŻNICY POMIĘDZY FULL A ZEROWY CONTEXT???

The drop in acc is from ... (for Swin) to ... (for MoCo) --może excluding Moco????




\begin{table}[ht!]
\caption{Deep Learning models' performance when full available contextual information is given.}
\begin{tabular}{ccccc}
\label{tab:metrics}
\textbf{model} & \textbf{accuracy} & \multicolumn{1}{l}{\textbf{precision}} & \textbf{recall} & \multicolumn{1}{l}{\textbf{AUC}} \\ \hline
\textit{ResNet18} & 0.8565 & 0.9500  & 0.7525 &  0.9420\\
\textit{DenseNet121} & 0.8745 & 0.9587 & 0.7825 & 0.9576 \\
\textit{Swin} & 0.9100  & 0.9745 & 0.8419 & 0.9729 \\
\textit{supViT} & 0.8995 & 0.9601 & 0.8335 & 0.9719  \\
\textit{MAE} & 0.9106 & 0.9609 & 0.8560 & 0.9753\\
\textit{MoCo} & 0.9051  & 0.9693 & 0.8367 & 0.9717
\end{tabular}
\end{table}



The global results were also analysed separately within the four groups: \textit{TP - True Positive, FP - False Positive, FN - False Negative, TN - True Negative}. The results for the model least sensitive to the limited amount of contextual information(\textit{Swin}) and most impacted convolutional model - \textit{ResNet18} are shown in Figure~\ref{fig:probs_4categories}.  It turns out that the mean probabilities within the groups do not change much with the limitation of the amount of contextual information. However, the number of images within the FN and TP groups changes significantly. It shows that the flows between the prediction for tumour lesions are bigger than for the normal tissues. Note that these fluctuations occurs for different context sizes for the two models. In general plots with the number of images within the four categories look similar for transformer-based models in a sense that FN and TP curves crosses only once but at different context sizes ({\color{red}from 14 in the case of \MoCo to 2 for \Swin}). 
%14 -moco, 8-vit, 4-mae, 2-swin (these are the last before the change)


%Due to the fact that in the case of transformer-based models, the context size is decreased by 3 pixels not by 1 pixel as in the case of convolutional models (see Section \textit{Image dimensions mapping}), the number of images undergoing a change of prediction at particular context size in the case of transformer-based model is divided by 3 to enable fair comparison with convolutional models. 


The issue is investigated in two scenarios (1) we take into account the images that changed their label more than once (referred to as \textit{'swinging images'}) (2) only the images that changed their label once.


%however, for \ResNet18 it looks similar. For transformer-based model, there were fewer data points (explained in Section on \textit{Image dimensions mapping}). 


\st{Moreover, the plots were more spare as often for given context size particular change of predictions were not observed. Interestingly, for models it is observed that the change of prediction occured either for the very small values of context size or the big once. For the moderate values, the change of predictions were relatively rarely observed. The summary of all the histograms corresponding to the models is provided in %Figure~\ref{fig:misleading_number}.
It is clearly seen that the model that most often changes (once) the decision about the image the most often is \MoCo. Interesting the mo }



%Lastly, it was analysed how many images in total experience by particular number of the changes of predictions given particular model (Figure~\ref{fig:misleading_number_all}). It turns out that even though the model that overall changes the predictions the most often in \DenseNet121, the models that in rare cases changes the predictions 



%We chose the black pixels as an indication of the removal of original image regions as this color is very rare in original data, unslike white color.




%for the first time at the given context size. 


{\color{blue}The results at a given context size means that it is the last `moment' before the change of prediction which happens given the next decreased context size.}


It turns out that indeed (as shown at Figure~\ref{fig:misleading_histogram}) in the case of \DenseNet121, the most changes occur for extreme context sizes but it is even more visible in the case of \ResNet18.


We divided the number of images per particular context size by 3 in the case of transformer-based models to account for the fact that we cut the size of the context in this case by 3 pixels not by 1 pixels as in the case of convolutional models



Due to the fact that 
We divided the number of images per particular context size by 3 in the case of transformer-based models to account for the fact that we cut the size of the context in this case by 3 pixels not by 1 pixels as in the case of convolutional models
 (see Section \textit{Image dimensions mapping})


 

As already seen (Table~\ref{tab:sensitive}, the model that overall changes the predictions the most often is \DenseNet121, the models that changes predictions even in 90\% of all possible context sizes is \MAE and \supViT. However, these are very rare - in the case of \MAE, there are only 4 such images, and in the case of \supViT - only one. Note that the area under the curves cannot be compared between the models from convolutional and transformer family as in the latter there are fewer data points. However, when comparing \DenseNet121 and \ResNet18, it is visible that for the \textit{`most swinging'} images the changes of predictions are more frequent in the case of \DenseNet121 than \ResNet18. The four \textit{`most swinging'} given \DenseNet121 are shown in Figure~\ref{fig:misleading}. The most similar models in behaviour are \supViT and \Swin.



The logarithm of the number of images that experience the change of prediction within a particular ratio of all possibilities to change by a particular model.






with the least confidence meaning that (1) we take the lowest probability of the two (if the~class 1 (tumour) is returned given two pixel values - 74\textsuperscript{th} and 75\textsuperscript{th}) or the highest probability from the two (if the class 0 (normal) is returned at least for one analysed pixel value). 


 if proper labels are provided


 (it is highlighted by the fact that the curves referring to the transformer-based models have markers)
